Pseudo-Physics-Informed Neural Operators: Enhancing Operator Learning from Limited Data

Neural operators have shown great potential in surrogate modeling. However, training a well-performing neural operator typically requires a substantial amount of data, which can pose a major challenge in complex applications. In such scenarios, detailed physical knowledge can be unavailable or difficult to obtain, and collecting extensive data is often prohibitively expensive. To mitigate this challenge, we propose the Pseudo Physics-Informed Neural Operator (PPI-NO) framework. PPI-NO constructs a surrogate physics system for the target system using partial differential equations (PDEs) derived from simple, rudimentary physics principles, such as basic differential operators. This surrogate system is coupled with a neural operator model, using an alternating update and learning process to iteratively enhance the model's predictive power. While the physics derived via PPI-NO may not mirror the ground-truth underlying physical laws -- hence the term ``pseudo physics'' -- this approach significantly improves the accuracy of standard operator learning models in data-scarce scenarios, which is evidenced by extensive evaluations across five benchmark tasks and a fatigue modeling application.

==> checklist.tex <==
\newpage
\section*{NeurIPS Paper Checklist}
\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} %\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: See the last a few sentences in the abstract and the last pargraph with the listed items in the introduction. 
 %A novel  Pseudo Physics-Informed Neural Operator (PPI-NO) framework constructs a  physics system using partial differential equations (PDEs) for the target system based on simple and naive physics knowledge such as basic differential operators.
% This approach significantly bolsters the accuracy and effectiveness of the state-of-the-art operator learning, especially in situations where the training data is limited in quantity.
%Under extensive evaluations  on five benchmark operator learning tasks, PPI-NO consistently outperforms the competitors by a significant margin.

    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{}
    %\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    % \item[] Justification: \justificationTODO{}
    \item[] Justification: See introduction part, ``The physics delineated by PPI-NO might not precisely reflect true physical phenomena...''; see Section~\ref{sect:limit} in the Appendix.
    %our findings reveal that this method markedly enhances the efficiency of operator learning, particularly with limited data quantity. In the future, we plan to develop more powerful neural networks that can learn a wider range of PDEs, and apply our method in more applications.
    
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{}
    %\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    % \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{}
    %\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: 
See the details of experiments in Appendix \ref{sect:detail}, and Section \ref{sect:expr}.

        
    % \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerNA{}
    
    %\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: 
We will provide open access to code and data after the reviewing process.

    % \justificat%ionTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{}
    
    %\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: 
See the beginning of Section \ref{sect:expr} where we clarify the training and testing details.

    % \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{}
    
    %\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
Justification:  See Table \ref{tab:advection} and Table \ref{tb:utof}
    where all the results were averaged from five runs and there were standard deviation to show the statistics of the experiments.

    
    % \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{}
    
    %\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: See the beginning of Section \ref{sect:expr} Line 254-255.

    
    
   % \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{}
    
    % \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    % \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerNA{}
    
    %\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
   % \item[] Justification: 

    %\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{}
    
    % \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our paper doesn't have such risks.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{}
    
    %\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We have cited the original paper about the models that we use.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented, and is the documentation provided alongside the assets?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    %\item[] Justification:  We will give an access to code later.

    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We do not have any experiments and research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our paper does not include any experiments and research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}

==> exp-old.tex <==

\section{Experiments}\label{sect:expr}
\noindent\textbf{Dataset.} We tested on five commonly used benchmark operator learning problems in literature~\citep{li2020fourier,lu2022comprehensive}, including \textit{Darcy Flow}, \textit{Nonlinear Diffusion}, \textit{Eikonal}, \textit{Poisson} and \textit{Advection}. The details are given in Section~\ref{sect:detail} of the Appendix. \zhe{In addition, we examined our method in one application in fatigue modeling. The task is to predict the stress intensity factor (SIF) for semi-elliptical surface cracks  on plates, given four geometric parameters that characterize the cracks~\citep{merrell2024stress}. The SIF plays a critical role in modeling crack growth by quantifying the stress state near the tip of a crack, and hence SIF computation and analysis is extremely important in fatigue modeling and fracture mechanics~\citep{anderson2005fracture}. The computation of SIF is expensive, because it typically needs to run finite element method (FEM) or extended FEM with very fine meshes~\citep{kuna2013finite}. 
Due to the complex sequence of computational steps involved in calculating SIFs, there is no holistic PDE that directly models the relationship between the geometric features and the SIF function. Instead, the computation of SIFs typically relies on numerical methods and the extraction of local stress fields near the crack tip.} 

 \noindent\textbf{Method and Settings.} We evaluated our method based on two popular NO models, FNO and DONet. For learning the pseudo physics laws via the neural network $\phi$ --- see \eqref{eq:pde-learn} --- we tuned the kernel size from \{(3, 3), (5, 5), (7, 7), (9, 9)\}. The stride was set to 1 and padding was set to ``same'' to ensure the output shape does not change. In the subsequent FNN, we chose the number of layers from \{3, 4, 5, 6\}, and the layer width from \{16, 32, 64\}. We used {GeLU} activation. For the cases of Darcy Flow, Eikonal and Poisson, we used the following derivatives $\{\partial_{x_1} u, \partial_{x_2} u, \partial_{x_1x_1}u, \partial_{x_2x_2}u, \partial_{x_1x_2} u\}$, and for the other cases, we used $\{\partial_x u, \partial_{xx} u, \partial_t u, \partial_{tt} u, \partial_{xt} u\}$. \zhe{SIF setting Keyan...}
For FNO, we set the number of modes to 12 and channels to 32 (in the lifted space). We varied the number of Fourier layers from \{2, 3, 4\}. For DONet, in all the cases except Darcy Flow,  the trunk net and branch net were constructed as FFNs. We varied the number of layers from \{2, 3, 4\} and the layer width was chosen from \{30, 40, 50, 60\}, with ReLU activation. For the case of Darcy flow, we found that DONet with only feed-forward layers exhibited inferior performance. To address this, we introduced convolution layers into the branch net. We selected the number of convolution layers from \{3,5,7\}, and employed batch normalization and leaky ReLU after each convolution layer.
To incorporate the learned pseudo physics representation into the training of FNO or DONet,  we randomly sampled 200 input functions to construct the second loss term in  \eqref{eq:fine-tune-loss}. 
We set the maximum number of iterations to $10$ and selected the weight $\lambda$ from $[10^{-1}, 10^{2}]$. 
All the models were implemented by PyTorch~\citep{paszke2019pytorch}, and optimized with ADAM~\citep{kingma2014adam}. The learning rate was selected from $\{10^{-4}, 5\times 10^{-4}, 10^{-3}\}$. The number of epochs for training or fine-tuning FNO, DONet and pseudo physics network $\phi$ was set to 500 to ensure convergence. 
For each operator learning benchmark, we simulated 100 examples for testing, and varied the number of training examples from \{5, 10, 20, 30\}, except for Advection, we ran with \{20, 30, 50, 80\} training examples. \zhe{For SIF prediction task (which is much more challening), we experimented with training size from \{400, 500, 600\}, and employed 100 test examples.}
We repeated the evaluation for five times, each time we randomly sampled a different training set. We ran experiments on workstations equipped with Nvidia Geforce RTX 4090 and Intel I9 CPU. 
%For each run, we first learned the standard FNO or DeepONet model based on the training data only. Then the model was fine-tuned (without any change on the model architecture) with the pseudo physics laws incorporated as in \eqref{eq:fine-tune-loss}. All the models were trained by ADAM optimization and the learning rate was tuned from $\{10^{-4}, 5\times 10^{-4}, 10^{-3}\}$. The number of epochs was to set 1000 to ensure convergence.  

\begin{table*}[t]
    \small
    \centering
    \begin{subtable}{\textwidth}
        \small 
        \centering
    \begin{tabular}{cccccc}
        \hline
        \textit{Training size}      &  & {5}             & {10}         & {20}     & {30}     \\ \hline
        FNO                  &  & 0.4915 $\pm$ 0.0210	& 0.3870 $\pm$ 0.0118   & 0.2783 $\pm$ 0.0212   & 0.1645 $\pm$ 0.0071         \\
        PPI-FNO          &  & {0.1716} $\pm$ {0.0048}          & {0.0956} $\pm$ {0.0084}        & {0.0680} $\pm$ {0.0031} 		 & {0.0642} $\pm$ {0.0010}    \\
        Error Reduction          &  & 65.08\% & 75.29\%        & 75.56\%		 & 60.97\%   \\ \hline
        DONet             &  & 0.8678 $\pm$ 0.0089          & 0.6854 $\pm$ 0.0363      & 0.5841 $\pm$ 0.0279 	& 0.5672 $\pm$ 0.0172    \\
        PPI-DONet             &  & 0.5214 $\pm$ 0.0543        & 0.3408 $\pm$ 0.0209    	& 0.2775 $\pm$ 0.0224	& 0.2611 $\pm$ 0.0084  \\ 
        Error Reduction  &  & 39.91\%         & 50.27\%    	& 52.49\%	& 53.96\%  \\ \hline
        % $\phi$-FNN             &  & 0.2585$\pm$ 0.0141          & 0.1819 $\pm$ 0.0026		& 0.1520  $\pm$ 0.0020	& 0.1413 $\pm$ 0.0013  \\
        % $\phi$          &  & 0.2285$\pm$ 0.0147         & 0.1392 $\pm$ 0.0080 	& 0.0898 $\pm$ 0.0046	& 0.0688 $\pm$ 0.0032  \\ \hline
    \end{tabular}
    \caption{\small \textit{Darcy flow}}
    \label{tab:darcy}
    \end{subtable}
    \begin{subtable}{\textwidth}
        \small
        \centering
        \begin{tabular}{cccccc}
        \hline
        \textit{Training size}      &  & {5}             & {10}         & {20}     & {30}     \\ \hline
        FNO                  &  & 0.2004 $\pm$ 0.0083	& 0.1242 $\pm$ 0.0046   & 0.0876 $\pm$ 0.0061   & 0.0551 $\pm$ 0.0021         \\
        PPI-FNO          &  & 0.0105 $\pm$ 0.0016         & 0.0066 $\pm$ 0.00023        & 0.0049 $\pm$ 0.00037 		 & 0.0038 $\pm$ 0.00039    \\
        Error Reduction          &  & 94.76\%         & 94.68\%        & 
        94.40\%		 & 93.10\%  \\
        \hline
        DONet             &  & 0.3010 $\pm$ 0.0119          & 0.2505 $\pm$ 0.0057      & 0.1726 $\pm$ 0.0076	& 0.1430 $\pm$ 0.0036    \\
        PPI-DONet             &  & 0.1478$\pm$ 0.0126          & 0.1161 $\pm$ 0.0124 	& 0.1032 $\pm$ 0.0059	& 0.0842 $\pm$ 0.0041  \\ 
        Error Reduction &  & 50.89\%         & 53.65\%    	& 40.20
        \%& 41.11\%  \\ \hline
        % $\phi$-FNN             &  & 0.0826$\pm$ 0.0070          & 0.0660 $\pm$ 0.0069  	& 0.0586  $\pm$ 0.0020	& 0.0463 $\pm$ 0.0022  \\
        % $\phi$            &  & 0.0303$\pm$ 0.0006         & 0.0233 $\pm$ 0.0005	& 0.0190 $\pm$ 0.0001	& 0.0163 $\pm$ 0.0002  \\ \hline
    \end{tabular}
    \caption{\small \textit{Nonlinear diffusion}}
    \end{subtable}
    \begin{subtable}{\textwidth}
    \small
    \centering
        \begin{tabular}{ccccc}
        \hline
        \textit{Training size}        & {5}             & {10}         & {20}     & {30}     \\ \hline
        FNO                    & 0.2102 $\pm$ 0.0133	& 0.1562 $\pm$ 0.0098   & 0.0981 $\pm$ 0.0022   & 0.0843 $\pm$ 0.0020        \\
        PPI-FNO            & 0.0678 $\pm$ 0.0026         & 0.0582 $\pm$ 0.0043        & 0.0493 $\pm$ 0.0023 		 & 0.0459 $\pm$ 0.0010    \\
        Error Reduction & 67.74\%         & 62.74\%        & 49.74\%		 & 45.55\%   \\
        \hline
        DONet               & 0.3374 $\pm$ 0.0944          & 0.1759 $\pm$ 0.0065      & 0.1191 $\pm$ 0.0047 	& 0.1096 $\pm$ 0.0037    \\
        PPI-DONet               & 0.1302$\pm$ 0.0127          & 0.0907 $\pm$ 0.0093 	& 0.0714 $\pm$ 0.0011	& 0.0700 $\pm$ 0.0007  \\ 
        Error Reduction   & 61.41\%         & 48.43\%    	& 40.05\%	& 36.13\%  \\ \hline
        % $\phi$-FNN               & 0.0192$\pm$ 0.0013          & 0.0144 $\pm$ 0.0009  	& 0.0072  $\pm$ 0.0004	& 0.0070$\pm$ 0.00005  \\
        % $\phi$             & 0.0153$\pm$ 0.0009         & 0.0108 $\pm$ 0.0006	& 0.0059 $\pm$ 0.0002	& 0.0052 $\pm$ 0.0002  \\ \hline
    \end{tabular}
    \caption{\small \textit{Eikonal}}
    \end{subtable}

    \begin{subtable}{\textwidth}
    \small 
    \centering
    \begin{tabular}{cccccc}
        \hline
        \textit{Training size}      &  & {5}             & {10}         & {20}     & {30}     \\ \hline
        FNO                  &  & 0.2340 $\pm$ 0.0083	& 0.1390 $\pm$ 0.0007   & 0.0895 $\pm$ 0.0008   & 0.0698 $\pm$ 0.0014         \\
        PPI-FNO          &  & {0.1437} $\pm$ {0.0062}          & {0.0771} $\pm$ {0.0018}        & {0.0544} $\pm$ {0.0009} 		 & {0.0458} $\pm$ {0.0003}    \\
        Error Reduction          &  & 38.59\% & 44.53\%        & 39.22\%		 & 34.38\%   \\ \hline
        DONet             &  & 0.6142 $\pm$ 0.0046          & 0.5839 $\pm$ 0.0090      & 0.5320 $\pm$ 0.0028 	& 0.5195 $\pm$ 0.0040    \\
        PPI-DONet             &  & 0.5275 $\pm$ 0.0037        & 0.5001 $\pm$ 0.0042    	& 0.4450 $\pm$ 0.0010	& 0.4258 $\pm$ 0.0040  \\ 
        Error Reduction  &  & 14.12\%         & 14.35\%    	& 16.35\%	& 18.04\%  \\ \hline
    \end{tabular}
    \caption{\small \textit{Poisson}}
    \label{tab:poisson}
    \end{subtable}
    \begin{subtable}{\textwidth}
        \small 
        \centering
    \begin{tabular}{cccccc}
        \hline
        \textit{Training size}      &  & {20}             & {30}         & {50}     & {80}     \\ \hline
        FNO                  &  & 0.4872 $\pm$ 0.0097	& 0.4035 $\pm$ 0.0086   & 0.3019 $\pm$ 0.0085   & 0.2482 $\pm$ 0.0059        \\
        PPI-FNO          &  & {0.3693} $\pm$ {0.0099}          & {0.3224} $\pm$ {0.0123}        & {0.2236} $\pm$ {0.0075} 		 & {0.1698} $\pm$ {0.0075}    \\
        Error Reduction          &  & 24.20\% & 20.10\%        & 25.94\%		 & 31.59\%   \\ \hline
        DONet             &  & 0.5795 $\pm$ 0.0045          & 0.4810 $\pm$ 0.0092      & 0.3882 $\pm$ 0.0086 	& 0.3164 $\pm$ 0.0072    \\
        PPI-DONet             &  & 0.3630 $\pm$ 0.0112        & 0.2897 $\pm$ 0.0097    	& 0.2629 $\pm$ 0.0053	& 0.2120 $\pm$ 0.0065  \\ 
        Error Reduction  &  & 37.36\%         & 39.77\%    	& 32.28\%	& 33.00\%  \\ \hline
    \end{tabular}
    \caption{\small \textit{Advection}}
    \label{tab:advection}
    \end{subtable}
    
    \caption{\small Relative $L_2$ error in five operator learning benchmarks, where ``PPI'' is short for Pseudo-Physics Informed''. $\phi$-FNN means only using FNN components to train the network $\phi$ (\ie removing the convolution layer). The last two rows of each table indicate the error in predicting the source function via $\phi$. All the results were averaged from five runs.  } \label{tb:all-pred-error}
\end{table*}

\subsection{Results and Analysis}\label{sect:exp-res}

%phi-performance


%learning curve & lambda
\begin{figure}
    \centering
    \setlength\tabcolsep{0pt}
	\begin{tabular}[c]{cccc}
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
\includegraphics[width=\textwidth]{iteration-learning-curve/darcy_flow_10_iteration_learning_curve.pdf}
        \caption{\small PPI-FNO: learning}\label{fig:fno-learning}
    \end{subfigure} & 
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
\includegraphics[width=\textwidth]{iteration-learning-curve/Nonlinear_diffusion_10_iteration_learning_curve_deeponet.pdf}
        \caption{\small PPI-DONet: learning}\label{fig:donet-learning}
    \end{subfigure} &
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
\includegraphics[width=\textwidth]{error-vs-lambda/darcy_flow_data_fno_error_vs_lam.pdf}
        \caption{\small PPI-FNO: $\lambda$}\label{fig:lambda-fno}
    \end{subfigure} &
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
\includegraphics[width=\textwidth]{error-vs-lambda/Nonlinear_diffusion_deeponet_error_vs_lam.pdf}
        \caption{\small PPI-DONet: $\lambda$} \label{fig:lam-donet}
    \end{subfigure}
    \end{tabular}
    \caption{\small Learning curve of PPI-FNO on Darcy Flow (a), and of PPI-DONet on nonlinear diffusion (b). In (c) and (d) we show how the weight $\lambda$ of ``pseudo physics'' affects the operator learning performance. The horizontal line in (c) and (d) are the relative $L_2$ errors of standard FNO and DONet. }
    \label{fig:learning-curve-and-lambda-study}
\end{figure}

\begin{table*}
    \small 
    \centering
    \begin{tabular}{ccccc}
        \hline
        \textit{Training size}      &  & {400}             & {500}         & {600}      \\ \hline
        FNO                  &  & 0.1776 $\pm$ 0.0150	& 0.1695 $\pm$ 0.0090   & 0.1122 $\pm$ 0.0094          \\
        PPI-FNO          &  & {0.1166} $\pm$ {0.0064}          & {0.1151} $\pm$ {0.0093}        &{0.0850}$\pm${0.0060} \\
        Error Reduction          &  & 34.35\% & 32.09\%        & 24.24\%		 \\ \hline
        DONet             &  & 0.5318 $\pm$ 0.0095          & 0.5155 $\pm$ 0.0200      & 0.4037 $\pm$ 0.0331 	  \\
        PPI-DONet             &  & 0.3490 $\pm$ 0.0034        & 0.3468 $\pm$ 0.0074    	& 0.3299 $\pm$ 0.0066	 \\ 
        Error Reduction  &  & 34.37\%         & 32.73\%    	& 18.28\%  \\ \hline
        % $\phi$-FNN             &  & 0.2585$\pm$ 0.0141          & 0.1819 $\pm$ 0.0026		& 0.1520  $\pm$ 0.0020	& 0.1413 $\pm$ 0.0013  \\
        % $\phi$          &  & 0.2285$\pm$ 0.0147         & 0.1392 $\pm$ 0.0080 	& 0.0898 $\pm$ 0.0046	& 0.0688 $\pm$ 0.0032  \\ \hline
    \end{tabular}
    \caption{\small SIF prediction for plate surface cracks in fatigue modeling.}
    \label{tab:crack}
    \end{table*}

\begin{figure}
	\centering
	\setlength\tabcolsep{0pt}
	\begin{tabular}[c]{cc}
	\begin{subfigure}[b]{0.48\textwidth}
		\centering
	\includegraphics[width=\textwidth]{./figs-deeponet/darcy/final_best_deep_five_darcy_5.pdf}
	\end{subfigure} &
    \begin{subfigure}[b]{0.48\textwidth}
		\centering
	\includegraphics[width=\textwidth]{./figs-fno/nl/final_best_five_nl_5.pdf}
	\end{subfigure}
 \\
	\begin{subfigure}[b]{0.48\textwidth}
		\centering
		\includegraphics[width=\textwidth]{./figs-deeponet/darcy/final_best_deep_five_darcy_10.pdf}
	\end{subfigure} &
 \begin{subfigure}[b]{0.48\textwidth}
		\centering
	\includegraphics[width=\textwidth]{./figs-fno/nl/final_best_five_nl_10.pdf}
	\end{subfigure}
 \\
 \begin{subfigure}[b]{0.48\textwidth}
		\centering
		\includegraphics[width=\textwidth]{./figs-deeponet/darcy/final_best_deep_five_darcy_20.pdf}
	\end{subfigure} &
 \begin{subfigure}[b]{0.48\textwidth}
		\centering
	\includegraphics[width=\textwidth]{./figs-fno/nl/final_best_five_nl_20.pdf}
	\end{subfigure}
 \\
 \begin{subfigure}[b]{0.48\textwidth}
		\centering
	\includegraphics[width=\textwidth]{./figs-deeponet/darcy/final_best_deep_five_darcy_30.pdf}
 \caption{\small \textit{PPI-DONet: Darcy Flow}}\label{fig:darcy-dont-example}
	\end{subfigure} & 
 \begin{subfigure}[b]{0.48\textwidth}
		\centering
	\includegraphics[width=\textwidth]{./figs-fno/nl/final_best_five_nl_30.pdf}
 \caption{\small \textit{PPI-FNO: nonlinear diffusion}}\label{fig:nl-fno-example}
	\end{subfigure}
\end{tabular}
	\caption{\small Examples of the prediction and point-wise error of PPI-DONet and PPI-FNO on \textit{Darcy Flow} and \textit{nonlinear diffusion}, respectively.  From top to bottom, the models were trained with 5, 10, 20, 30 examples.}
 \vspace{-0.2in}
\end{figure}

\noindent\textbf{Predictive performance.} 
We reported the average relative $L_2$ error and the standard deviation (before and after incorporating the pseudo physics laws) in Table \ref{tb:all-pred-error}. The model trained with the learned physics laws (see \eqref{eq:fine-tune-loss}) is denoted as PPI-FNO or PPI-DONet, short for Pseudo Physics Informed FNO/DONet.
In all cases, with our pseudo physics informed approach , the prediction error of both FNO and DONet experiences a large reduction. For instance, across all training sizes in \textit{Darcy Flow} and \textit{nonlinear diffusion}, PPI-FNO reduces the relative $L_2$ error of the ordinary FNO by over 60\% and 93\%, respectively. In \textit{Darcy Flow} with training sizes 10 to 30, PPI-DONet reduces the error of the ordinary DONet by over 50\%. Even the minimum reduction across all cases achieves 14.12\% (PPI-DONet over DONet on \textit{Poisson} with training size 5). 

Together these results demonstrate the strong positive impact of the learned physics by our neural network model $\phi$ specified in Section \ref{sect:phi}. Although it remains opaque and non-interpretable, it encapsulates valuable knowledge that greatly enhances the performance of operator learning, in particular with limited data.

 
Next, we assessed the accuracy of the learned physics laws by examining the relative \(L_2\) error in predicting the source functions \(f\) from \(\phi\) (see \eqref{eq:pde-learn}). We tested on \textit{Darcy Flow}, \textit{nonlinear diffusion}, and \textit{Eikonal}. We compared a baseline method that removes the convolution layer of \(\phi\), leaving only the feed-forward layers. 
The average relative \(L_2\) error and standard deviation are reported in Table \ref{tb:utof}. It can be observed that in nearly every case, adding a convolution layer indeed significantly improves the accuracy of \(\phi\). This improvement might be attributed to the convolution layer's ability to integrate neighboring information and compensate for the error introduced by the numerical difference in approximating  the derivatives. We also experimented with multiple convolution layers, but the improvement was found to be marginal. 
%\begin{table}

\begin{wraptable}{r}{0.65\textwidth}
\small
\centering
\begin{subtable}{0.6\textwidth}
   \small
    \centering
    \begin{tabular}{ccc}
    \hline \textit{Benchmark} & FNN & Ours \\
    \hline
    Darcy Flow & 0.1819$\pm$0.0026 & \textbf{0.1392$\pm$ 0.0080}\\
    Nonlinear Diffusion & 0.0660$\pm$0.0069 & \textbf{0.0233$\pm$0.0005}\\
    Eikonal & 0.0144$\pm$0.0009 & \textbf{0.0108 $\pm$ 0.0006}\\
    \hline
    \end{tabular}
    \caption{\small Training size=10}
\end{subtable}
\begin{subtable}{0.6\textwidth}
   \small
    \centering
    \begin{tabular}{ccc}
    \hline \textit{Benchmark} & FNN & Ours \\
    \hline
    Darcy Flow & 0.1413$\pm$0.0013 & \textbf{0.0688$\pm$ 0.0032}\\
    Nonlinear Diffusion & 0.0463$\pm$0.0022 & \textbf{0.0163$\pm$0.0002}\\
    Eikonal & 0.0070$\pm$0.00005 & \textbf{0.0052 $\pm$ 0.0002}\\
    \hline
    \end{tabular}
    \caption{\small Training size=30}
\end{subtable}
\caption{\small Relative $L_2$ error of using the learned back-box PDE network~\eqref{eq:pde-learn} to predict the input function. } \label{tb:utof}
%\end{table}
\end{wraptable}

In addition, we also found the operator learning improvement is relatively \textit{robust} to the accuracy of our physics representation $\psi$. For instance, on \textit{Darcy Flow} with training size 5 and 10, the relative $L_2$ error of $\phi$ network is 0.2285 and 0.1392, which is significantly bigger than with training size 30  where the relative $L_2$ error is 0.0688. Yet the error reduction upon FNO (see Table~\ref{tab:darcy}) under all the three training sizes is above 60\%. The error reduction upon DONet is 40\% for training size 5 and over 50\% for training size 10 and 30. 
The results imply that even roughly capturing the underlying physics (with $\phi$) can substantially boost the operator learning performance.   


Third, we examined the learning behavior of our method, which conducts an iterative, alternatingly fine-tuning process. We employed one \textit{Darcy Flow}, one \textit{nonlinear diffusion} and one \textit{Eikonal} dataset, each with 30 examples. We show the test relative $L_2$ error along with the iterations in Fig. \ref{fig:fno-learning}, \ref{fig:donet-learning}, and Appendix Fig.~\ref{fig:fno-learning-eikonal} and Fig.~\ref{fig:donet-learning-eikonal}. As we can see, the predictive performance of our algorithm kept improving and tended to converge at last, affirming the efficacy of the learning process. 


\noindent\textbf{Point-wise prediction and point-wise error.} For a detailed assessment, we conducted a fine-grained evaluation by visualizing the predictions and point-wise errors made by each method. In Fig. \ref{fig:darcy-dont-example} and \ref{fig:nl-fno-example},  we showcased the predictions and point-wise errors using PPI-DONet for \textit{Darcy Flow}, PPI-FNO for \textit{nonlinear diffusion}, respectively. Additional examples of predictions and point-wise errors are provided in Fig. \ref{fig:ek-fno-example}, \ref{fig:ek-deeponet-example}, \ref{fig:darcy-fno-example}, and \ref{fig:nl-deeponet-example} in the Appendix.
 
It is evident that without the assistance of the pseudo physics laws learned by our method, the ordinary DONet and FNO frequently missed crucial local structures, sometimes even learning entirely incorrect structures.
For example, In Fig. \ref{fig:darcy-dont-example} the first row, DONet missed one mode, while in the second and third row of Fig. \ref{fig:darcy-dont-example}, DONet failed to capture all the local modes. 
After incorporating the learned physics, DONet (now denoted as PPI-DONet; see the third column) successfully captures all the local modes, including their shapes and positions. Although not all the details are exactly recovered, the point-wise error is substantially reduced, particularly in those high error regions of the ordinary DONet; see the fourth column of Fig. \ref{fig:darcy-dont-example}.

In another instance, as shown in Fig. \ref{fig:nl-fno-example}, where the ordinary FNO (second column) captured the global shape of the solution, but the mis-specification of many local details led to large point-wise errors across many regions (fourth column). In contrast, PPI-FNO (third column) not only identified the structures within the solution but also successfully recovered the details. As a result, the point-wise error (fifth column) was close to zero everywhere.

Additional instances can be found in Fig. \ref{fig:ek-fno-example}, the first three rows illustrate that ordinary FNO (trained with 5, 10, and 20 examples, respectively) estimates an entirely incorrect structure of the solution, indicating that the training data is insufficient for FNO to capture even the basic structure of the solution. In contrast, after fine-tuning with our learned physics laws from the same sparse data, PPI-FNO accurately figured out the solution structures and yielded a substantial reduction in point-wise error across nearly everywhere. The point-wise error became uniformly close to zero.
With 30 examples, the ordinary FNO was then able to capture the global structure of the solution, but the details in the bottom left, bottom right, and top right corners were incorrectly predicted. In comparison, PPI-FNO further recovered these details accurately. 




Collectively, these results demonstrate that the pseudo physics extracted by our method not only dramatically boosts the overall prediction accuracy but also better recovers the local structures and details of the solution.

\textbf{Real World Data Experiments.} \keyan {
We also tested our learning framework on a real-world dataset.%explaination of the crack dataset%
Since the real data will be much more complex than the previous physics PDE equations, we choose to use training examples from {400,500,600}. Following the experiment before, we still evaluated the real-world dataset on FNO and DONet(see Table~\ref{tab:crack}). These results also demonstrate our learning framework's positive feasibility and positive impact on real-world data.

}

\textbf{Ablation study.} \keyan {In addition, in the ablation study, we first verify the effectiveness of our PDE network $\phi$. Specifically, we tested on the Darcy-flow benchmark with alternative choices of $\phi$, including (1) a standard FNO where the input is $u$ and the output is $f$, and (2)  a pixel-wise MLP with the same number of layers and width as in our method, where the input is $u$ value at a grid point, and the output is the corresponding $f$ value at that grid point.  The relative $L_2$ error in predicting $f$ of each method is given(see Table~\ref{tb:phierror}). It shows that our design of $\phi$ with $u$ derivatives indeed outperforms other architectures, showing the effectiveness of learning a (black-box) PDE representation.

\begin{table*}[t]
\small
\centering
\begin{subtable}{\textwidth}
   \small
    \centering
    \begin{tabular}{ccccc}
    \hline \textit{Training size} & 5 & 10 & 20 & 30 \\
    \hline
    FNO & 0.7229$\pm$0.0318 & 0.5759$\pm$ 0.0126 & 0.4257$\pm$ 0.0106 & 0.3160$\pm$ 0.0037\\
    MLP & 0.7169$\pm$0.0160 & 0.6598$\pm$ 0.0056 & 0.6464$\pm$ 0.0029 & 0.6277$\pm$ 0.0032\\
    Ours & \textbf{0.2285 $\pm$ 0.0147} & \textbf{0.1392 $\pm$ 0.0080} & \textbf{0.0898 $\pm$ 0.0046} & \textbf{0.0688 $\pm$ 0.0032}\\
    \hline
    \end{tabular}
    \caption{\small Error of predicting $f$}
\end{subtable}
\begin{subtable}{\textwidth}
   \small
    \centering
    \begin{tabular}{ccccc}
    \hline \textit{Training size} & 5 & 10 & 20 & 30 \\
    \hline
    PPI-FNO with FNO as $\phi$ & 0.5853$\pm$0.0153 & 0.3871$\pm$ 0.0124 & 0.2613$\pm$ 0.0190 & 0.1629$\pm$ 0.0064\\
    PPI-FNO with MLP as $\phi$ & 0.7262$\pm$0.0920 & 0.5516$\pm$ 0.0699 & 0.4568$\pm$ 0.0857 & 0.3983$\pm$ 0.1051\\
    Standard FNO & 0.4915 $\pm$ 0.0210	& 0.3870 $\pm$ 0.0118   & 0.2783 $\pm$ 0.0212   & 0.1645 $\pm$ 0.0071\\
    Ours & \textbf{0.1716 $\pm$ 0.0048} & \textbf{0.0956 $\pm$ 0.0084} & \textbf{0.0680 $\pm$ 0.0031} & \textbf{0.0642 $\pm$ 0.0010}\\
    \hline
    \end{tabular}
    \caption{\small PPI training of operator $f\rightarrow u$, test error}
\end{subtable}
\caption{\small The relative $L_2$ error in predicting $f$ of each method } \label{tb:phierror}
%\end{table}
\end{table*}

We also investigate the performance of $\phi$ regarding the choice of derivatives. Specifically, we tested our PPI-FNO on the Darcy-flow cases and varied the order of derivatives up to 0, 1, 2, and 3. Note in our paper, we used the order up to 2(see Table~\ref{tb:ordererror}). We observed that although the accuracy of $\phi$ with derivatives up to the third order is slightly better than with derivatives up to the second order, the best operator learning performance was still achieved using derivatives up to the second order. This might be because higher-order derivative information can cause overfitting in the PDE network $\phi$ to a certain degree. Such higher-order information may not be critical to the actual mechanism of the physical system and can therefore impede the improvement of operator learning performance.

\begin{table*}[t]
\small
\centering
\begin{subtable}{\textwidth}
   \small
    \centering
    \begin{tabular}{ccccc}
    \hline \textit{Training size} & 5 & 10 & 20 & 30 \\
    \hline
    order 0 & 0.7126$\pm$0.0131 & 0.5733$\pm$0.0208 & 0.4812$\pm$0.0399 & 0.3445$\pm$0.0182 \\ 
    order $\le$ 1 & 0.2926$\pm$0.0118 & 0.2006$\pm$0.0047 & 0.1379$\pm$0.0051 & 0.1084$\pm$0.0053 \\ 
    order $\le 2$ (ours) & \textbf{0.2285$\pm$0.0147} & \textbf{0.1392$\pm$0.0080} & \textbf{0.0898$\pm$0.0046} & \textbf{0.0688$\pm$0.0032} \\ 
    order $\le 3$ & 0.2058$\pm$0.0192 & 0.1123$\pm$0.0039 & 0.0712$\pm$0.0021 & 0.0585$\pm$0.0030 \\ 
    \hline
    \end{tabular}
    \caption{\small The error of black-box PDE network $\phi$ (i.e., $u\rightarrow f$)}
\end{subtable}
\begin{subtable}{\textwidth}
   \small
    \centering
    \begin{tabular}{ccccc}
    \hline \textit{Training size} & 5 & 10 & 20 & 30 \\
    \hline
    order 0 & 0.6352$\pm$0.0673 & 0.4523$\pm$0.0621 & 0.3570$\pm$0.0658 & 0.2737$\pm$0.0643 \\ 
    order $\le$ 1 & 0.3386$\pm$0.0259 & 0.2161$\pm$0.0083 & 0.1645$\pm$0.0114 & 0.1197$\pm$0.0132 \\ 
    order $\le 2$ (ours) & \textbf{0.1716$\pm$0.0048} & \textbf{0.0956$\pm$0.0084} & \textbf{0.0680$\pm$0.0031} & \textbf{0.0642$\pm$0.0010} \\ 
    order $\le 3$ & 0.2959$\pm$0.0381 & 0.1719$\pm$0.0213 & 0.1193$\pm$0.0158 & 0.0828$\pm$0.0054 \\ 
    \hline
    \end{tabular}
    \caption{\small The corresponding operator learning error (i.e., $f \rightarrow u$)}
\end{subtable}
\caption{\small The relative $L_2$ error in predicting $f$ of each order } \label{tb:ordererror}
%\end{table}
\end{table*}
}


Finally, we examined the effect of the weight $\lambda$ of our ``pseudo physics''; see \eqref{eq:ppi-loss}. To this end, we used one \textit{Darcy Flow} dataset and \textit{nonlinear diffusion} dataset with training size 30. We varied $\lambda$ from $[0.5, 10^2]$, and run PPI-FNO and PPI-DONet on \textit{Darcy Flow} and \textit{nonlinear diffusion}, respectively. As shown in Fig.~\ref{fig:lambda-fno} and~\ref{fig:lam-donet}, we can see that across a wide range of $\lambda$ values, PPI-FNO and PPI-DONet can consistently outperform the standard FNO and DONet respectively by a large margin. However, the choice $\lambda$ does have a significant influence on the operator learning performance, and the best choice is often in between. In Appendix Fig.~\ref{fig:lambda-fno-eikonal} and~\ref{fig:lam-donet-eikonal}, we show results on \textit{Ekonal}, which we obtain similar observations. 


\textbf{Time and Memory Analysis.} \keyan {The alternative training process requires more training cycles than standard NO, but the time complexity only grows linearly with the number of alternating iterations, not quadratically or exponentially. We believe this is reasonable and practically acceptable.
For memory analysis, Our "pseudo" physics network $\phi$ is very small as compared to standard neural operators (NO) --- $\phi$ is simply a pixel-wise MLP coupled with one convolution filter, resulting in a marginal increase in memory cost. The below shows under training size = 30, the parameter count of FNO, DONet and their pseudo physics informed version. On average, PPI-FNO increases the number of parameters over FNO by 1.29 while PPI-DONet by DONet increases by 1.89.(see Table~\ref{tb:paracounts})

\begin{table*}[t]
\small
\centering
\begin{tabular}{ccccc}
\hline
\textbf{Parameter count} & \textbf{FNO} & \textbf{PPI-FNO (increase)} & \textbf{DONet} & \textbf{PPI-DONet (increase)} \\ 
\hline
Darcy-flow & 1188353 & 1229476 (+3.46\%) & 2084704 & 2125827 (+1.97\%) \\ 
Nonlinear-diffusion & 1188353 & 1197220 (+0.75\%) & 824501 & 833368 (+1.08\%) \\ 
Eikonal & 1188353 & 1197220 (+0.75\%) & 824501 & 833368 (+1.08\%) \\ 
Poisson & 1188353 & 1197220 (+0.75\%) & 824501 & 833368 (+1.08\%) \\ 
Advection & 1188353 & 1197220 (+0.75\%) & 210101 & 218968 (+4.22\%) \\ 
\hline
\end{tabular}
\caption{\small Parameter counts for FNO and DONet with PPI variations across different problems } \label{tb:paracounts}
\end{table*}
}

==> method-old.tex <==
\section{Background}
\noindent\textbf{Problem Formulation.} Operator learning seeks to approximate an operator that maps input parameters and/or functions to corresponding output functions.  
%Operator learning, an emergent field in machine learning, focuses on learning mappings between infinite-dimensional spaces, primarily aiming to discover and approximate unknown operators. 
In most practical cases, operator learning rises in the context of solving partial differential equations (PDEs), where the operator corresponds to the solution operator of the PDE.
Assume a PDE system:
\begin{equation}
	\label{eq:pde}
	% \mathcal{N}u(\x) = f(\x), \quad \x \in \Omega
	% \mathcal{N}[u](\mathbf{x}, t) = f(\mathbf{x}, t), \quad \mathbf{x} \in \Omega \times [0,\infty) 
	\mathcal{N}[u](\mathbf{x}) = f(\mathbf{x}), \quad \mathbf{x} \in \Omega \times [0,\infty), 
\end{equation}
where $\x$ is a compact notation for the spatial and temporal coordinates, $\Omega$ is the spatial domain, $[0,\infty)$ is the temporal domain, $\mathcal{N}$ is a nonlinear differential operator, $u(\mathbf{x})$ is the solution function, and $f(\mathbf{x})$ is the source term. Solving the PDE system is to find the solution function $u(\mathbf{x})$ that satisfies the PDE system equation \eqref{eq:pde} as well as the initial and boundary conditions. This task often necessitates the use of computationally expensive numerical solvers such as finite element method (FEM) or finite difference method (FDM). To alleviate the computational challenge, we aim to learn the solution operator of the PDE system, \({\psi}: \mathbb{F} \rightarrow \mathbb{U}\) using a training dataset \(\mathcal{D} = \{(\f_n,\u_n)\}_{n=1}^N\), which consists of discretized functions $u(\x)$ and $f(\x)$ at a set of collocations points. Once the operator model is trained, it can be used to directly predict the solution function $u$ for new instances of the input $f$,   offering a much more efficient alternative to running numerical solvers from scratch. However, the training dataset still needs to be generated offline using numerical solvers.


\cmt{
Our objective is to learn a function-to-function mapping \({\psi}: \mathbb{F} \rightarrow \mathbb{U}\), where \(\mathbb{F}\) and \(\mathbb{U}\) represent two function spaces (e.g., Banach spaces) using a training dataset \(\mathcal{D} = \{(\f_n,\u_n)\}_{n=1}^N\) that consists of discretized $u(\x)$ and $f(\x)$ at a set of collocations points. % $\{\x_1, \x_2, \cdots, \x_{m}\}$. 
% and $\{\x'_1, \x'_2, \cdots, \x'_{m'} \}$, respectively.
Directly working with the functional space is often infeasible. Thus, classic operator learning learns a mapping between the discretized input and output functions, %$\psi: \mathbb{R}^m \rightarrow \mathbb{R}^{m'}$, i.e., 
\ie $\psi(\f) = \u$, where $\f$ and $\u$ are the values of $f$ and $u$ sampled at the collocation points, respectively.  
%$\f = [f(\x_1), f(\x_2), \cdots, f(\x_m)]^\top$ and $\u = [u(\x'_1), u(\x'_2), \cdots, u(\x'_{m'})]^\top$.
}


\noindent\textbf{Fourier Neural Operator (FNO)}
~\citep{li2020fourier} represents a significant leap in neural network architecture for operator learning, especially in solving PDEs. For a given discretized input function \(\f\), FNO first employs a feed-forward network (FFN) on each component of \(\f\) at its respective sampling location, thereby lifting the input into a higher-dimensional channel space. The core of FNO is the Fourier layer, which performs a linear transformation followed by a nonlinear activation within the functional space,  
$ h(\mathbf{x}) \leftarrow \sigma \left( \mathcal{W}h(\mathbf{x}) + \int \kappa(\mathbf{x} - \mathbf{x}')h(\mathbf{x}')d\mathbf{x}' \right)$, where \(h(\mathbf{x})\) is the input to the Fourier layer, \(\kappa(\cdot)\) the integration kernel, and \(\sigma(\cdot)\) the activation function. The convolution operation in this context is efficiently computed using the convolution theorem:
$ \int \kappa(\mathbf{x} - \mathbf{x}')h(\mathbf{x}')d\mathbf{x}' = \mathcal{F}^{-1} [\mathcal{F}[\kappa] \cdot \mathcal{F}[h]](\mathbf{x})$, 
where \(\mathcal{F}\) and \(\mathcal{F}^{-1}\) denote the Fourier and inverse Fourier transforms, respectively. The Fourier layer's efficiency stems from performing the Fast Fourier Transform (FFT) on \(h\), multiplying it with the discretized kernel in the frequency domain, and then applying the inverse FFT. The local linear transformation, \(\mathcal{W}h(\mathbf{x})\), is executed through conventional convolution operations. After multiple Fourier layers, the final output is obtained by the channel-wise application of another FFN, projecting the representation back to the original space.

\noindent\textbf{Deep Operator Network (DONet)}~\citep{lu2021learning}, is another prominent work in operator learning. %Conceptualized on the universal approximation theorem for operators, DONets are capable of approximating any continuous linear or nonlinear operator under certain conditions. 
The architecture of a DONet is  structured into two primary components: the branch network and the trunk network, learning representations for the input functions and querying locations, respectively. 
Consider an input function \(f(\x) \in \mathbb{F}\) evaluated at \(m\) sensor locations \(\{\x_1, \x_2, \cdots, \x_m\}\) and an output function \(u \in \mathbb{U}\).
The branch network receives the values \([f(\x_1), f(\x_2), \cdots, f(\x_m)]\) and outputs a feature representation \([b_1, b_2, \cdots, b_p]^\top \in \mathbb{R}^p\). Concurrently, the trunk network processes a querying location $\x$
and outputs another feature vector \([t_1, t_2, \cdots, t_p]^\top \in \mathbb{R}^p\).
The approximation of the output function \(u(\x)\) is then computed as a sum of products of the corresponding elements from the branch and trunk networks, $\mathcal{G}[f](\x) \approx \sum_{k=1}^p b_k t_k$,
 % \begin{equation}
 % 	\label{eq:deeponet}
 % 	\mathcal{G}[f](\x) \approx \sum\nolimits_{k=1}^p b_k t_k,
 % \end{equation} 
where \(\mathcal{G}\) is the learned operator mapping input function \(f\) to the corresponding output function  \(u\).
% where \(G\) is the operator mapping input function \(f\) to the corresponding output function \(G(f)\).
% Here, \(G\) denotes the DeepONet operator that takes an input function \(f\) and produces an output function \(G(f)\), approximated at the points \(\y\).

%This architecture allows DONet to learn complex mappings between infinite-dimensional spaces. However, similar to other frameworks, DONet faces challenges in data acquisition, especially in scenarios where training data is scarce and costly to obtain.

\textbf{Physics-Informed Neural Operator (PINO)}~\citep{wang2021learning,li2021physics}  has recently emerged as a promising approach to address the data scarcity issue in operator learning.
% In recent years, physics-informed neural operators (PINO) have emerged as a promising approach to address the data scarcity issue in operator learning. PINO leverages the governing physical equations as soft constraints during the training process to guide the learning of the neural operator.
%In an effort to mitigate these challenges, the concept of Physics-Informed Neural Operators (PINO)~\citep{wang2021learning,li2021physics} has been introduced. 
PINO embeds physical laws, \eg governing equations, directly into the learning process, serving as soft constraints that guide the training of the model. The incorporation of physical principles not only enhances the model's adherence to ground-truth phenomena but also reduces its dependency on extensive training data. 
%PINO operates by assimilating physical equations, typically in the form of partial differential equations (PDEs), into the neural network's architecture. This approach ensures that the learned operator not only fits the training data but also respects the underlying physical laws governing the system. For example, in a PINO model designed for fluid dynamics, the Navier-Stokes equations might be integrated into the training process to enforce the alignment of the fluid behavior with established physical principles.
Mathematically, the integration of physics into the learning process can be viewed as an additional regularization term in the loss function. Let \(\mathcal{L}_\text{data}\) represent the traditional data-fitting loss term (\eg the mean squared error between predicted and actual outputs), the physics-informed term \(\mathcal{L}_\text{physics}\) can be the residual of the governing PDEs evaluated at the neural network's outputs. The total loss function \(\mathcal{L}\) for a PINO model is then expressed as
\[ \mathcal{L} = \mathcal{L}_\text{data} + \lambda \mathcal{L}_\text{physics}, \]
where \(\lambda\) is a weighting factor that balances the importance of data-fitting versus physics compliance. This approach encourages the model to learn solutions that are not only consistent with the provided data but also physically plausible.



\section{Methodology}
In the absence of the underlying physics knowledge (\ie the PDE system \eqref{eq:pde} is not available), it is impossible to construct the physics loss term in the PINO framework.
To address this challenge, we propose a ``pseudo'' physics-informed operator learning framework motivated by the need to uncover the underlying physical laws using available data. This approach is particularly useful in complex, challenging applications, where data is often costly or sparse while the underlying physics is hard to fully understand. 	
%To address the challenge of operator learning with sparse data in real-world scenarios, 
%we propose a framework motivated by the need to uncover the underlying physical laws using available data. This approach is particularly relevant in fields like climate modeling, where data is often costly or sparse while the underlying physics is hard to fully understand. 	
Our model architecture is depicted in Figure \ref{fig:model}.

% In the second step, we learn the mapping $\psi: f \rightarrow u$ with initial sparse data. Then we sample many new $f'$ data from a given distribution, and utilize the mapping learned with sparse data to predict corresponding $u'$ such that $\psi(f')=u'$. After that, based on the mapping $\phi: u \rightarrow f$ learned in the first step, we use $u'$ to reconstruct $f'$. Then we use the reconstruction loss w.r.t $f'$ and training data loss to fine tune the mapping $\psi: f \rightarrow u$ so that the performance of operator learning with sparse data could improve.

% 
% \subsection{Motivation}

% There are many implict physics laws in the system, and it is significant to use the data available to find the underlying physical laws so that people can have an access to learn, understand, and create in the system.

% Existing operator learning methods often suppose that the data used to train the model is sufficient which means that the physical laws are learned fully from data. However, in the real world such as power system, autonomous driving, the data is always costly or sparse which results in the difficulty of operator learning in many cases. Therefore there exists a question:

% \textbf{Given sparse data, can we firstly discover some underlying physical laws and then improve the performance of operator learning?}
% Based on this question, we propose a two-step framework to improve the operator learning with sparse data.

% \subsection{Overall Framework}
\subsection{Pseudo Physics System Learning}\label{sect:phi}
As the first step, we propose a novel approach to learn the physics system using sparse training data. 
Our key observation is that, \textit{although the mapping from $f$ to $u$ can be intricate and may necessitate information across the entire domain (in theory, $u$ is an integration of the Green's function multiplied with $f$ over the domain), the underlying PDE system \eqref{eq:pde} simplifies to a local combination of $u$ and its derivatives.} We therefore use a neural network $\phi$ to approximate the general form of $\N$, 
\begin{align}
    \N[u](\x) \approx \phi\left(\x, u(\x), S_1(u)(\x), \ldots, S_Q(u)(\x)\right), \label{eq:pde-learn}
\end{align}
where  $\{S_j\}_{j=1}^Q$ are $Q$  derivative operators that we believe should be present in the system, such as $\partial_t u$, $\partial_{tt} u$, $\partial_{x_1} u$, $\partial_{x_2} u$,  
$\partial_{x_1x_1} u$, $\partial_{x_1x_2} u$, $\partial_{x_2x_2}u$, and more. 

%The local combination nature of the PDE representation decouples the values of $u$ and its derivatives across different sampling locations, and thereby dramatically increase the number of training data points. For example, suppose the input function $f$ and output function $u$ are sampled at a $128 \times 128$ grid. A single pair of the discretized input and output functions, $(\f, \u)$ is typically far from sufficient for a neural operator to learn the mapping $f\rightarrow u$. However, this sample can be decoupled into $128\times 128 = 16,384$ training data points to learn $\phi$ as in \eqref{eq:pde-learn}. Hence we can expect that even with sparse training examples for operator learning, the learning of the PDE system $\Ncal$ via our formulation \eqref{eq:pde-learn}
%can still be accurate, due to a relatively much larger number of training data points can be decoupled from these training examples.


The inherent local combination nature of the PDE representation decouples the values of $u$ and its derivatives across various sampling locations, thereby significantly increasing the number of available training data points. For instance, consider sampling the input function $f$ and output function $u$ on a $128 \times 128$ grid. A single pair of discretized input and output functions, denoted as $(\f, \u)$, is typically insufficient for a neural operator to effectively learn the mapping $f \rightarrow u$. However, this sample can be decomposed into $128 \times 128 = 16,384$ training data points to train $\phi$ as outlined in \eqref{eq:pde-learn}. Consequently, even with sparse training examples for operator learning, the learning of the PDE system $\mathcal{N}$ via our formulation in \eqref{eq:pde-learn} can still achieve accuracy, thanks to the much greater number of training data points that can be derived from these examples.

\begin{figure*}[t]
    \centering
    \setlength\tabcolsep{0pt}
    \includegraphics[width=0.8\textwidth]{./model.pdf}
    %\vspace{-0.1in}
    \caption{\small The illustration of the Pseudo Physics-Informed Neural Operator (PPI-NO). At the top, a black-box PDE representation is learned through the neural network $\phi$. At the bottom, the acquired ``pseudo'' physics laws are utilized to construct a reconstruction loss, thereby regulating the NO training.
    %Step 1 learns a black-box PDE representation via the neural network $\phi$. In Step 2, the learned ``pseudo'' physics laws is used to construct a reconstruction loss, regularizing the NO training. 
    } \label{fig:model}
\end{figure*}

We use an $L_2$ loss to estimate the parameters of $\phi$, which is defined as 
\begin{align}
	\Lcal_\phi =  \sum\nolimits_{n=1}^{N}\sum\nolimits_{j=1}^M &\left[\phi(\x_{j}, u_n(\x_{j}), S_1(u_n)(\x_{j}), \ldots, S_Q(u_n)(\x_{j})) - f_n(\x_{j})\right]^2, \label{eq:eq-loss}
\end{align}
where $f_n(\cdot)$ and $u_n(\cdot)$ are the input and output functions in $n$-th training example, and $\{\x_1, \ldots \x_M\}$ are the  locations at which we discretize $f_n$ and $u_n$. 

% For a dynamic system, we could use the steady state data to learn the mapping $\phi: u \rightarrow f$ and then use the learned mapping to predict the dynamic data generated by the pseudo system using simulations with initial condition $u_0(\x)$ and boundary condition $\mathcal{B}(\x)$.
% The training loss function is defined as:
% \begin{align}
% 	\label{eq:loss}
% 	\mathcal{L}(\pmb{\upsilon}) = 
% \frac{1}{N} \sum_{n=1}^{N} \left| \phi\left(\pmb{\upsilon}, \u, {\u_x}_n, {\u_{xx}}_n, {\u_t}_n, {\u_{tt}}_n \right)- \f_n \right|^2,
% \end{align}
% where  $N$ is the number of training data, $\u$ is the discretized representation of function $u(\x)$ at collocation point , ${\u_x}_n$, ${\u_{xx}}_n$, ${\u_t}_n$, ${\u_{tt}}_n$ are the discretized representation of function $u_x$, $u_{xx}$, $u_t$, $u_{tt}$ at collocation point, $\f_n$ is the discretized representation of function $f(\x)$ at collocation points.

We use numerical difference to obtain the derivatives of each $u_n$, namely, $S_k(u_n)$ ($1 \le k \le Q$), and then feed these inputs to the neural network $\phi$ to compute the prediction. 
As the numerical difference method may introduce errors when calculating derivatives, we incorporate a convolution layer in $\phi$ to collect and integrate neighborhood information about $u$ and its numerical derivatives, aiming to compensate for these errors. After that, we use feed-forward layers to sequentially perform linear transforms and nonlinear activation to obtain the prediction at each sampling location; see Fig. \ref{fig:model} top. The learned neural network mapping $\phi: u \rightarrow f$, although black-box in nature,
encapsulates crucial physics knowledge inherent in the data employed for operator learning. %(even such data can be sparse)

%In some complex systems, we might only have steady-state data despite the system is dynamic. In such cases, we can instead model $u_t$ using the neural network $\phi$. Since at the steady state, we have $u_t = 0$, we fit each $\phi(\x_j, u_n(\x_j), S_1(u_n)(\x_j), \ldots, S_Q(u_n)(\x_j))$ to zero in \eqref{eq:eq-loss}.




% To solve this PDE, boundary conditions (BCs) and initial conditions (ICs) are necessary. These can be expressed as:
% Boundary Conditions: \( \mathcal{B}[u](\mathbf{x}, t) = g(\mathbf{x}, t), \quad \mathbf{x} \in \partial\Omega \)
% ; Initial Conditions: \( u(\mathbf{x}, 0) = u_0(\mathbf{x}), \quad \mathbf{x} \in \Omega \),
% where \(\mathcal{B}\) is an operator defining the boundary conditions on the boundary \(\partial\Omega\) of the domain, \(g(\mathbf{x}, t)\) specifies the boundary values, and \(u_0(\mathbf{x})\) is the initial state of the system.





% Implicit Physics Learning here aims to learn the underlying physical laws from sparse data based on the estimation of derivatives for $u$.


\subsection{Coupling Neural Operator with Pseudo Physics}
Next, we leverage the pseudo physics laws embedded in the learned mapping \(\phi: u \rightarrow f\) to enhance the neural operator learning process. Specifically, we use \(\phi\) to reconstruct \(f\) from the \(u\) predicted by the neural operator. % that learns to maps from $f$ to $u$. 
In this way, our approach goes beyond relying solely on the training data; it uses the physics laws learned in the previous step to incorporate a reconstruction error into optimizing the neural operator parameters. %mapping \(\psi: f \rightarrow u\).

%which is obtained using the mapping \(\psi: f \rightarrow u\) trained with sparse data. This approach goes beyond relying solely on sparse data; instead, it uses the physics laws learned in the previous step for reconstructing \(f\) from \(u\) and incorporates the reconstruction error into optimizing the mapping \(\psi: f \rightarrow u\).

Initially, we train the neural operator \(\psi: f \rightarrow u\) using the available training data, creating a preliminary model. This model is developed using FNO or DONet or their variants. The focus is to first establish a fundamental understanding of the relationship between \(f\) and \(u\), based on the limited data. Next, the loss function for \(\psi\) is augmented using the physics laws learned in the first step, %$\mathcal{L}=  \sum_{n=1}^{N} \mathcal{L}_2(\psi(f_n),u_n) + \lambda \cdot  \EE_{p(f')} \left[\mathcal{L}_2(f', \phi(\psi(f')))\right]$,
\begin{align}
 	\mathcal{L}=  \sum\nolimits_{n=1}^{N} \mathcal{L}_2(\psi(f_n),u_n) + \lambda \cdot  \EE_{p(f')} \left[\mathcal{L}_2(f', \phi(\psi(f')))\right], \label{eq:ppi-loss}
 \end{align}
where the first term is the \(\mathcal{L}_2\) loss for data fitting (as in the standard neural operator training), and the second term is the expected reconstruction error for the input function.  %newly sampled data related to the physics-informed loss. 
The second term incorporates the physics laws embedded in $\phi(\cdot)$, and \(\lambda\) is a weight factor that balances the training data loss against the reconstruction error.

%In practice, \(f'\) denotes data sampled from the distribution of \(f\), and \(\phi(\psi(f'))\) is the reconstruction of \(f'\) using the learned mappings \(\phi\) and \(\psi\). These samples can be generated using Gaussian processes with a radial basis function kernel. The computation of the integral in the loss function is approximated using Monte Carlo sampling:
In practice, the expected reconstruction error does not have a closed form. One can sample a collection of $f'$ from the underlying distribution of the input function $p(\cdot)$, \eg a Gauss random field or Gaussian process, and then employ a Monte-Carlo approximation, 
\begin{align}
	\mathcal{L}=  \sum_{n=1}^{N} \mathcal{L}_2(\psi(f_n),u_n) + \lambda  \frac{1}{N'} \sum_{n=1}^{N'} \mathcal{L}_2(f'_n, \phi(\psi(f'_n))), \label{eq:fine-tune-loss}
\end{align}
where \(N'\) is the number of input function samples. % from the distribution of \(f\).



% **Iterative Refinement and Fine-Tuning:**
%\todo{@shandian: need to clarify.}

To enhance the operator learning process, the model is iteratively refined. In each iteration, we first fine-tune the neural operator $\psi$ with the pseudo physics $\phi$ fixed, and then fix $\psi$,  fine-tune  $\phi$ to refine the physics representation. This fine-tuning loop is carried out for multiple iterations, allowing for continuous improvement of the neural operator based on the refined physics.
%After fine-tuning the \(\psi: f \rightarrow u\) model for specific epochs, we use the updated model to make more precise predictions of \(u'\) than initially possible.
%This fine-tuning loop continues for multiple iterations, allowing for the continuous improvement of the neural operator based on the refined physics.


This methodology mirrors  human experts' approach to physics system modeling, where sparse data is used to learn the physics laws inspired by simple differential operation (up to the 2nd order to imitate human experts), and then these laws are utilized to generalize the system for data generation. The  reconstruction loss term augments the operator learning with additional information, leading to potential improvement upon only training with sparse data. 
% \Keyan{
% \subsection{Alternative training with Pseudo Physics Regularization}
% In this step, we propose an alternative training method to help enhance our neural operator performance. Generally, it uses a similar method to improve \(\phi: u \rightarrow f\) and then improve the neural operator \(\psi: f \rightarrow u\) by using the enhanced \(\phi: u \rightarrow f\). We can cycle-enhance both models to improve their performance.

% We first follow a similar procedure in section 3.2 to enhance the learned mapping  \(\phi: u \rightarrow f\). Particularly, we reuse the expected reconstruction error for the input function, but we use the $\phi(\cdot)$ in section 3.2 to define our first term in the loss function,
% \begin{align}
% 	\mathcal{L}=  \sum_{n=1}^{N} \mathcal{L}_2(\phi(u_n),f_n) + \lambda  \frac{1}{N'} \sum_{n=1}^{N'} \mathcal{L}_2(f'_n, \phi(\psi(f'_n))), \label{eq:fine-tune-loss}
% \end{align}
% where the first term is the \(\mathcal{L}_2\) loss for physics laws learned in section 3.1, and the second term is the reused expected reconstruction error for the input function in section 3.2. 

% We then use the improved mapping \(\phi: u \rightarrow f\) to reprocess section 3.2 again. We produce the modeling as an alternative training method and try to make the neural operator, and the physics laws we learned can enhance each other.
% }


% In order to accelerate the process of operator learning, after fine tuning the networks for $\psi: f \rightarrow u$ in specific epochs, we can use the updated preliminary model to predict the corresponding $u'$ which are more precise than the values the initial preliminary model predicts. We continue this fine tuning loop for 10 episodes. (\todo{not sure what paragraph means.})

% Augmented operator learning here aims to accelerate and improve the performance of operator learning with sparse data based on the physics learned in the first step. With the physics learned in our framework, operator learning with sparse data could achieve similar performance compared with operator learning with sufficient training data.  (\todo{not sure what paragraph means.})

% \todo{rewrite this section}
% \subsection{Neural Operator with Physics Regularization}
% Once we learn the pseudo physics laws thorough the implicit mapping $\phi: u \rightarrow f$, we use the learned mapping $\phi$ to reconstruct $f$ from $u$ which is leaning using the mapping $\psi: f \rightarrow u$ trained with sparse data.
% In stead on solely relying on the sparse data, we use the physics laws learned in the first step to reconstruct $f$ from $u$ and use the reconstruction error as a part of optimizing the mapping $\psi: f \rightarrow u$.

% % Then we use the reconstruction loss w.r.t $f'$ and training data loss to fine tune the mapping $\psi: f \rightarrow u$ so that the performance of operator learning with sparse data could improve.

% % More specifically, we firstly train a neural operator $\psi: f \rightarrow u$ using the initial sparse data and get a preliminary model. The mapping $\psi: f \rightarrow u$ is trained by FNO and modified DeepONet in this article.
% % When training branch networks, we introduce only one branch network. Regardless of the specific positions of input function $f$, we flatten the grid coordinates and make the predictions of embedding vectors $[b_1, b_2, \cdots, b_k]$ for each sample.



% % In order to perform operator learning with sparse data, it is natural to think that we try to generate more data pairs based on the physics laws we have learned in the first step and the distribution information of source terms. 
% More specifically, we firstly train a mapping $\psi: f \rightarrow u$ using the original sparse data and get a preliminary model. The mapping $\psi: f \rightarrow u$ is trained by FNO and modified DeepONet in this article.
% % 

% Similar to the PINN, the loss function $\psi$ is augmented using the physics laws learned in the first step. The loss function is defined as:
% % \begin{align}
% % 	\mathcal{L}=  \mathcal{L}_2(\psi(f),u) + \lambda  \mathcal{L}_2(f', \phi(\psi(f'))),
% % \end{align}
% \begin{align}
% 	\label{eq:loss}
% 	\mathcal{L}=  \sum_{n=1}^{N} \mathcal{L}_2(\psi(f_n),u_n) + \lambda  \int_{f'} \mathcal{L}_2(f', \phi(\psi(f'))) p(f') \d f',
% \end{align}
% where the first term in R.H.S is the $\mathcal{L}_2$ loss corresponding to sparse data, the second term in R.H.S is the error for reconstruction of sampled new data related to physics informed loss. In this second term, it includes the physics laws we learned in the first step of our framework. $\lambda$ determines the weights of reconstruction error from new generated data compared with sparse training data loss.
% In this equation, $f'$ denoted collection data sampled from the distribution of $f$ and $\phi(\psi(f'))$ is the reconstruction of $f'$ using the learned mapping $\phi$ and $\psi$. Such samples can be generated using Gaussian process with radial basis function kernel \citep{rasmussen2006gaussian} combined with the physics laws learned in the first step. 
% In practice, the computation of the integral in the second term of the loss function is approximated using Monte Carlo sampling. i.e.,
% \begin{equation}
% 	\label{eq:loss}
% 	\mathcal{L}=  \sum_{n=1}^{N} \mathcal{L}_2(\psi(f_n),u_n) + \lambda  \frac{1}{N} \sum_{n=1}^{N'} \mathcal{L}_2(f'_n, \phi(\psi(f'_n))),
% \end{equation}
% where $N'$ is the number of samples from the distribution of $f$.


% % sampled from a given distribution and $\phi(\psi(f'))$ is the reconstruction of $f'$ using the learned mapping $\phi$ and $\psi$.


% % When training branch networks, we introduce only one branch network.
% % Regardless of the specific positions of input function $f$, we flatten the grid coordinates and make the predictions of embedding vectors $[b_1, b_2, \cdots, b_k]$ for each sample. 
% % Then we replicate the embedding vectors for each grid points and let the output of branch network multiply with the output of trunk network to get the final prediction of $u$ at search points.

% % After training a preliminary model, we sample $f'$ which follows the same distribution of $f$ in the dataset from radial-basis function kernel using gaussian process, and feed $f'$ to the preliminary trained model to predict $u'$, then use implicit physics model trained in the first step to reconstruct $f'$. 
% % 

% % Since the preliminary model mapping $\psi: f \rightarrow u$ is trained only with sparse data, the reconstruction of $f'$ here is not so accurate. 
% % We use this error as a part of optimizing the preliminary model which maps from $f$ to $u$. 

% The idea here is similar to auto-encoder where the target is to learn two models such that given an input, it can automatically produce the input without labels. 
% This process imitate the process of physics system modeling by human experts where the sparse data is used to learn the physics laws that is described by a concise PDE system. 
% Then the learned physics laws are then extracted to generalize the physics system to generate more data.
% Considering the model inadquacy, we introduce the weights $\lambda$ to balance the reconstruction error and the sparse data loss.
% This can be interpreted as a kind of data augmentation where prior knowledge of physics laws learned from sparse data is used to generate more data to improve the performance of operator learning while keeping our data fitting task as the primary goal.


% The difference in our model is that we only optimize parameters of $\psi: f \rightarrow u$ and set the parameters of $\psi: f \rightarrow u$ freeze since in the first step with the information from neighbors and their estimations of derivative values for $u$, the physics behind $u \rightarrow f$ have been well-learned. The loss function to fine tune mapping $\psi: f \rightarrow u$ in Augmented Operator learning is defined as 
% \begin{align}
	% \mathcal{L}=  \mathcal{L}_2(\psi(f),u) + \lambda  \mathcal{L}_2(f', \phi(\psi(f')))
% \end{align}
% where the first term in R.H.S is the $\mathcal{L}_2$ loss corresponding to sparse data, the second term in R.H.S is the error for reconstruction of sampled new data related to physics informed loss. In this second term, it includes the physics laws we learned in the first step of our framework. $\lambda$ determines the weights of reconstruction error from new generated data compared with sparse training data loss. 





% \subsection*{PINN}
% In the context of PINNs, the solution \(u(\mathbf{x}, t)\) is approximated by a neural network \(\hat{u}(\mathbf{x}, t; \boldsymbol{\theta})\). The goal is to train this network such that it satisfies the PDE, along with the boundary and initial conditions. The loss function for this task typically includes three parts:

% 1. PDE Residual Loss:
% \[ \mathcal{L}_{PDE}(\boldsymbol{\theta}) = \frac{1}{N_p} \sum_{i=1}^{N_p} \left|\mathcal{N}[\hat{u}](\mathbf{x}_i, t_i; \boldsymbol{\theta}) - f(\mathbf{x}_i, t_i)\right|^2 \]
% 2. Boundary Condition Loss:
%    \[ \mathcal{L}_{BC}(\boldsymbol{\theta}) = \frac{1}{N_b} \sum_{j=1}^{N_b} \left|\mathcal{B}[\hat{u}](\mathbf{x}_j, t_j; \boldsymbol{\theta}) - g(\mathbf{x}_j, t_j)\right|^2 \]
% 3. Initial Condition Loss:
%    \[ \mathcal{L}_{IC}(\boldsymbol{\theta}) = \frac{1}{N_i} \sum_{k=1}^{N_i} \left|\hat{u}(\mathbf{x}_k, 0; \boldsymbol{\theta}) - u_0(\mathbf{x}_k)\right|^2 \]

% where \(N_p\), \(N_b\), and \(N_i\) are the number of collocation points used for enforcing the PDE, boundary conditions, and initial conditions, respectively.

% % **Optimization:**
% The training process involves adjusting the neural network parameters \(\boldsymbol{\theta}\) to minimize the combined loss:
% \[ \mathcal{L}(\boldsymbol{\theta}) = \mathcal{L}_{PDE}(\boldsymbol{\theta}) + \mathcal{L}_{BC}(\boldsymbol{\theta}) + \mathcal{L}_{IC}(\boldsymbol{\theta}). \]
% This optimization ensures that the network \(\hat{u}(\mathbf{x}, t; \boldsymbol{\theta})\) not only approximates the solution of the PDE but also satisfies the specified boundary and initial conditions, effectively embedding the physics of the problem into the neural network model.

